SplitBrain: Hybrid Data and Model Parallel Deep Learning

The recent success of deep learning applications has coincided with those widely available powerful computational resources for training sophisticated machine learning models with huge datasets. Nonetheless, training large models such as convolutional neural networks using model parallelism (as opposed to data parallelism) is challenging because the complex nature of communication between model shards makes it difficult to partition the computation efficiently across multiple machines with an acceptable trade-off. This paper presents SplitBrain, a high performance distributed deep learning framework supporting hybrid data and model parallelism. Specifically, SplitBrain provides layer-specific partitioning that co-locates compute intensive convolutional layers while sharding memory demanding layers. A novel scalable group communication is proposed to further improve the training throughput with reduced communication overhead. The results show that SplitBrain can achieve nearly linear speedup while saving up to 67\% of memory consumption for data and model parallel VGG over CIFAR-10.

==> Makefile <==
# Makefile for the Paper

SRC=$(shell ls *.tex styles/*.sty *.bib sections/*.tex)

default: pdf

pdf: main.pdf 

main.dvi: $(SRC)
	cd figures; make pdf; cd -
	latex main
	bibtex main
	latex main
	latex main
	rm -f *.log *.aux *.blg *.cb *.out *.bbl

#main.pdf: main.dvi	
#	dvipdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 -dEmbedAllFonts=true -dSubsetFonts=true -dMonoImageResolution=600 -dMaxSubsetPct=100 main.dvi main.pdf
#	rm -f *.log *.aux *.blg *.cb *.out *.bbl

main.pdf: $(SRC)
	cd figures; make pdf; cd -
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main
#	rm -f *.log *.aux *.blg *.cb *.out *.bbl

 
diff.pdf: $(SRC)
	cd figures; make pdf; cd -
	pdflatex diff 
	bibtex diff 
	pdflatex diff 
	pdflatex diff 
#	rm -f *.log *.aux *.blg *.cb *.out *.bbl

clean:
	rm -f *.cb *.cb2 *.bak *.bbl *.blg *.log *.aux *.ps *.dvi *.pdf *.out \
		sections/*.bak

